Quantitative Linear Logic for Neuro-Symbolic Learning and Verification

Differentiable Logics are deployed in neuro-symbolic learning tasks as a way of embedding logical constraints in the training objective of neural networks. A differentiable logic consists of a syntax to write logical properties and a semantics to interpret them as real-valued functions to be folded in the loss function. A defining trade-off of the field is that between logical properties of the connectives, and analytic concerns for the semantics, with both aspects being relevant in applications. At one extreme we find fuzzy logics, that have well-established algebraic and proof-theoretic foundations, and at the other ad-hoc differentiable logics like Fischer's DL2, conceived for deep learning applications. However, no satisfactory foundation has emerged yet. We propose a resolution to this long-standing tension via a novel logic, Quantitative Linear Logic (QLL), with foundational ambitions. Our design is driven by naturality -- the idea that, since logical constraints are translated to losses, the semantics of the connectives should be pertinent operations used in ML practice (that is, sum and log-sum-exp) on additive quantities (like logits). We then judge the result on two aspects: logical adequacy -- that they satisfy most of the standard logical laws of Linear Logic; and empirical effectiveness -- test-time performance (as measured by adversarial attacks) is well-correlated to the actual verification of the logical constraints (as measured by off-the-shelf neural network verifiers), which makes QLL stand out among SoTA techniques.

==> Definitions.tex <==
%% ----------------------------------------------------------------
%% Definitions.tex
%% ---------------------------------------------------------------- 
\RequirePackage{mathtools}
\RequirePackage{xparse}
\RequirePackage{pgffor}
\RequirePackage{ifthen}
\RequirePackage{amssymb}
\RequirePackage{xspace}


\newcommand{\BibTeX}{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

%% People
\newcounter{address}
\setcounter{address}{1}
\renewcommand{\theaddress}{\textsuperscript{\fnsymbol{address}}}
\newcommand{\address}[1]{\refstepcounter{address}\theaddress#1\\}
\newcommand{\Name}[3]{\texorpdfstring{\href{mailto:#3}{#2}#1}{#2}\xspace}
\newcommand{\SteveRGunn}[1]{\Name{#1}{Steve R. Gunn}{S.R.Gunn@ecs.soton.ac.uk}}

%% Dingbats
\newcommand{\tick}{\ding{51}}
\newcommand{\cross}{\ding{55}}

%% Calculus
\newcommand{\pd}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}\xspace}
\newcommand{\fd}[2]{\ensuremath{\frac{d #1}{d #2}}\xspace}
\newcommand{\dint}{\ensuremath{\int\!\!\!\int}\xspace}
\newcommand{\tint}{\ensuremath{\int\!\!\!\int\!\!\!\int}\xspace}

%% Math Sets
\newcommand{\Q}[1]{\ensuremath{\mathbb{#1}}\xspace}
\newcommand{\R}{\Q{R}}

%% Matrix, Vector
\newcommand{\V}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
\newcommand{\M}[1]{\ensuremath{\boldsymbol{#1}}\xspace}
\newcommand{\0}{\V{0}}
\newcommand{\1}{\V{1}}
\newcommand{\I}{\M{I}}

%% Math Functions
\newcommand{\F}[1]{\ensuremath{\mathrm{#1}}\xspace}
\newcommand{\sgn}{\F{sgn}}
\newcommand{\tr}{\F{trace}}
\newcommand{\diag}{\F{diag}}

%% Math Names
\newcommand{\N}[1]{\ensuremath{\mathit{#1}}\xspace}

%% Data
\newcommand{\mc}[1]{\ensuremath{\mathcal{#1}}\xspace}
\newcommand{\Hyp}{\mc{H}}
\newcommand{\D}{\mc{D}}

%% Kernel
\newcommand{\K}{\M{K}}
\newcommand{\eins}{\texorpdfstring{\ensuremath{\epsilon}}{\textepsilon}-insensitive\xspace}
\newcommand{\e}{\ensuremath{\epsilon}\xspace}
\newcommand{\Bxi}{\ensuremath{\boldsymbol{\xi}}\xspace}
\newcommand{\Kanova}{\ensuremath{\mathit{K_{ANOVA}}}\xspace}
\newcommand{\Kspline}{\ensuremath{\mathit{K_{spline}}}\xspace}

%% Bayesian
\newcommand{\MP}{\ensuremath{\mathit{{\scriptscriptstyle \hspace{-1.5pt}M\hspace{-1.5pt}P}}}\xspace}
\newcommand{\ML}{\ensuremath{\mathit{{\scriptscriptstyle \hspace{-1.5pt}M\hspace{-1.5pt}L}}}\xspace}
\newcommand{\Qw}{\ensuremath{Q_{\w}(\w)}\xspace}
\newcommand{\Qa}{\ensuremath{Q_{\Ba}(\Ba)}\xspace}
\newcommand{\Qb}{\ensuremath{Q_{\beta}(\beta)}\xspace}
\newcommand{\wMPab}{\ensuremath{\w_{\MP|\bar {\Ba},\bar \beta}}\xspace}
\newcommand{\wMP}{\ensuremath{\w_{\MP}}\xspace}
\newcommand{\yMP}{\ensuremath{y_{\MP}}\xspace}
\newcommand{\BaMP}{\ensuremath{\Ba_{\hspace{1pt}\MP}}\xspace}
\newcommand{\aMP}{\ensuremath{\alpha_{\hspace{1pt}\MP}}\xspace}
\newcommand{\bMP}{\ensuremath{\beta_{\hspace{1pt}\MP}}\xspace}
\newcommand{\Sab}{\ensuremath{\M{\Sigma}_{\bar \Ba,\bar \beta}}\xspace}
\newcommand{\Ba}{\ensuremath{\boldsymbol{\alpha}}\xspace}
\newcommand{\Bb}{\ensuremath{\boldsymbol{\beta}}\xspace}
\newcommand{\Bm}{\ensuremath{\boldsymbol{\mu}}\xspace}
\newcommand{\BL}{\ensuremath{\boldsymbol{\Lambda}}\xspace}
\newcommand{\BPhi}{\ensuremath{\boldsymbol{\Phi}}\xspace}
\newcommand{\SMP}{\ensuremath{\M{\Sigma}_{\MP}}\xspace}

\newcommand{\Pa}{\ensuremath{P(\alpha|\mathcal{H})}\xspace}
\newcommand{\Pb}{\ensuremath{P(\beta|\mathcal{H})}\xspace}
\newcommand{\Pab}{\ensuremath{P(\alpha,\beta|\mathcal{H})}\xspace}
\newcommand{\Pw}{\ensuremath{P(\w|\mathcal{H})}\xspace}
\newcommand{\PD}{\ensuremath{P(\D|\mathcal{H})}\xspace}
\newcommand{\PwIa}{\ensuremath{P(\w|\alpha,\mathcal{H})}\xspace}
\newcommand{\PDIwb}{\ensuremath{P(\D|\w,\beta,\mathcal{H})}\xspace}
\newcommand{\PDwab}{\ensuremath{P(\D,\w,\alpha,\beta|\mathcal{H})}\xspace}
\newcommand{\PDIw}{\ensuremath{P(\D|\w,\mathcal{H})}\xspace}
\newcommand{\PwID}{\ensuremath{P(\w|\D,\mathcal{H})}\xspace}
\newcommand{\PwabID}{\ensuremath{P(\w,\alpha,\beta|\D,\mathcal{H})}\xspace}

\newcommand{\PanH}{\ensuremath{P(\alpha)}\xspace}
\newcommand{\PbnH}{\ensuremath{P(\beta)}\xspace}
\newcommand{\PabnH}{\ensuremath{P(\alpha,\beta)}\xspace}
\newcommand{\PwnH}{\ensuremath{P(\w)}\xspace}
\newcommand{\PDnH}{\ensuremath{P(\D)}\xspace}
\newcommand{\PwIanH}{\ensuremath{P(\w|\alpha)}\xspace}
\newcommand{\PDIwbnH}{\ensuremath{P(\D|\w,\beta)}\xspace}
\newcommand{\PDwabnH}{\ensuremath{P(\D,\w,\Ba,\beta)}\xspace}
\newcommand{\PDIwnH}{\ensuremath{P(\D|\w)}\xspace}
\newcommand{\PwIDnH}{\ensuremath{P(\w|\D)}\xspace}
\newcommand{\PwabIDnH}{\ensuremath{P(\w,\alpha,\beta|\D)}\xspace}

\newcommand{\PDwBab}{\ensuremath{P(\D,\w,\Ba,\beta|\mathcal{H})}\xspace}
\newcommand{\PwIBa}{\ensuremath{P(\w|\Ba,\mathcal{H})}\xspace}
\newcommand{\PBab}{\ensuremath{P(\Ba,\beta|\mathcal{H})}\xspace}
\newcommand{\PwBabID}{\ensuremath{P(\w,\Ba,\beta|\D,\mathcal{H})}\xspace}

\newcommand{\PBanH}{\ensuremath{P(\Ba)}\xspace}
\newcommand{\PwIBanH}{\ensuremath{P(\w|\Ba)}\xspace}

%% Snakes
\newcommand{\Esnake}{\ensuremath{\mathit{E_{snake}}}\xspace}
\newcommand{\Eimage}{\ensuremath{\mathit{E_{image}}}\xspace}
\newcommand{\Econt}{\ensuremath{\mathit{E_{cont}}}\xspace}
\newcommand{\Ecurv}{\ensuremath{\mathit{E_{curv}}}\xspace}
\newcommand{\Eint}{\ensuremath{\mathit{E_{int}}}\xspace}
\newcommand{\Eext}{\ensuremath{\mathit{E_{ext}}}\xspace}
\newcommand{\Eterm}{\ensuremath{\mathit{E_{term}}}\xspace}
\newcommand{\Eline}{\ensuremath{\mathit{E_{line}}}\xspace}
\newcommand{\Eedge}{\ensuremath{\mathit{E_{edge}}}\xspace}
\newcommand{\Econ}{\ensuremath{\mathit{E_{con}}}\xspace}
\newcommand{\Eangle}{\ensuremath{\mathit{E_{angle}}}\xspace}
\newcommand{\Elshape}{\ensuremath{\mathit{E_{lshape}}}\xspace}
\newcommand{\Eedgedir}{\ensuremath{\mathit{E_{edgedir}}}\xspace}
\newcommand{\Emodel}{\ensuremath{\mathit{E_{model}}}\xspace}
\newcommand{\wte}{\ensuremath{\mathit{w_{term}}}\xspace}
\newcommand{\wli}{\ensuremath{\mathit{w_{line}}}\xspace}
\newcommand{\wed}{\ensuremath{\mathit{w_{edge}}}\xspace}
\newcommand{\wco}{\ensuremath{\mathit{w_{con}}}\xspace}

%% Environments
\newcounter{alg}
\newenvironment{algorithm}[1]
{
    \stepcounter{alg}
    \begin{table}[htb]
    \centering
    \begin{tabular}[t]{ll}
    \hline&\\
    \multicolumn{2}{l}{\bf Algorithm \arabic{alg}: #1}\\&\\
} {
    &\\
    \hline
    \end{tabular}
    \end{table}
}

%basic symbols maths
\newcommand{\Real}{{\mathbb R}}
%\newcommand{\terms}{{\mathcal{T}}}
\newcommand{\domainSymbol}{{\mathcal{D}}}
\newcommand{\distr}{p}
\newcommand{\dataset}{\mathcal{X}}
\newcommand{\hypothesis}{\mathcal{H}}
%\newcommand{\property}{\phi}
\newcommand{\logic}{L}
\newcommand{\godel}{G\"{o}del}
\newcommand{\Bool}{\mathbb{B}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\id}{x}
\newcommand{\val}{a}
\newcommand{\cons}[2]{#1 :: #2}
\newcommand{\consNew}[2]{#2[#1]}

%% comments 
\newcommand{\TODO}{{\color{red} \textbf{TODO}}}
\newcommand{\yada}{{\color{red} \textbf{yada yada }}}
\newcommand{\mcita}{{\color{red} \textbf{??}}}
\newcommand{\jnote}[2][]{\todo[color=black!10,#1]{JAIRO: #2}}
%\newcommand{\knote}[2][]{\todo[inline,color=blue!10,#1]{KK: #2}}
%\newcommand{\enote}[2][]{\todo[inline,color=teal!10,#1]{Enrico: #2}}
%\newcommand{\anote}[2][]{\todo[inline,color=orange!10,#1]{AB: #2}}

%% Keywords
\newcommand{\AI}[0]{AI}
\newcommand{\AILong}[0]{Artificial Intelligence}
\newcommand{\SiAI}{Symbolic \AI}
\newcommand{\SiAILong}{Symbolic \AILong}
\newcommand{\SuAI}{Subsymbolic \AI}
\newcommand{\SuAILong}{Subsymbolic \AILong}
\newcommand{\InAI}{Intersymbolic \AI}
\newcommand{\InAILong}{Intersymbolic \AILong}
\newcommand{\NN}{Neural Network}
\newcommand{\nn}{neural network}
\newcommand{\QL}{Quantitative Logic}
\newcommand{\DL}{Differentiable Logic} 
\newcommand{\mathcomp }[0]{\emph{MathComp}}
\newcommand{\OurLogic}[0]{Quantitative Linear Logic}
\newcommand{\OL}[0]{QLL}

% classes of Numbers
\newcommand{\real}[0]{\mathbb{R}}
\newcommand{\nat}[0]{\mathbb{N}}
\newcommand{\ereal}[0]{\overline{\real}}
\newcommand{\Ereal}[0]{[-\infty,\infty]}
\newcommand{\PEreal}[0]{[0,\infty]}

%Extended Reals 
\newcommand{\ldual}[1]{ #1 ^\bot}
\newcommand{\edual}[1]{ #1 ^{-1}}
\newcommand{\conmul}[0]{\otimes}
\newcommand{\por}[1]{\lor^{#1}}
\newcommand{\limp}[0]{\Rightarrow}
\newcommand{\dismul}[0]{\,\rotatebox[origin=c]{180}{\&}\,}
\newcommand{\pand}[1]{\land^{#1}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\sigmal}[1]{\Sigma_{#1}}
\newcommand{\LMS}[3]{\int^{#2}_{#3} #1}
\newcommand{\LM}[2]{\int^{#2} #1}
\newcommand{\esup}[1]{\mathrm{ess}\, \sup\,(#1)}
\newcommand{\einf}[1]{\mathrm{ess}\, \inf\,(#1)}
%\newcommand{\sigmal}[1]{\Sigma_{#1}}
\newcommand{\prob}[1]{\mathbb{P}(#1)}

%logic
%\newcommand{\neutral}{\textbf{0}}
\newcommand{\wetu}{\textbf{t}}
\newcommand{\stfa}{\textbf{f}}
\newcommand{\tempty}[1]{\llbracket #1 \rrbracket}
\newcommand{\m}[2][p]{\llbracket #2 \rrbracket_#1}
\newcommand{\bm}[2][\boolReal]{\llbracket #2 \rrbracket_{\mathrm{Bool}}^{#1}}
\newcommand\sepimp{\mathrel{-\mkern-6mu*}}
%\newcommand{\ldual}[1]{ #1 ^{\bot}}

%Horn 
\newcommand{\goal}{\mathcal{Q}}
\newcommand{\definite}{\mathcal{P}}
\newcommand{\atom}{\mathcal{A}}
\newcommand{\atome}{A}
\newcommand{\gatom}{\mathcal{A}_{\goal}}
\newcommand{\datom}{\mathcal{A}_{\definite}}
%quantifiers
\newcommand{\lforall}[3]{\forall #1 : #2\ldotp #3}
\newcommand{\lexists}[3]{\exists #1 : #2\ldotp #3}
\newcommand{\pforall}[4]{\forall^{#1}(#2 \in #3)\ldotp #4}
\newcommand{\pexists}[4]{\exists^{#1}(#2 \in #3)\ldotp #4}

% High-level language
\newcommand{\FunType}[2]{\ensuremath{#1 \text{ $ \rightarrow $ } #2}}
%\newcommand{\App}[2]{\ensuremath{#1 \text{ $ \rightarrow $ } #2}}
\newcommand{\VecType}[1]{\ensuremath{\text{Vec } #1}}
\newcommand{\FinType}[1]{\ensuremath{\text{Index } #1}}
\newcommand{\BoolType}{\ensuremath{\text{Bool}}}
\newcommand{\RealType}{\ensuremath{\text{Real}}}
\newcommand{\PRealType}{\ensuremath{\text{PReal}}}

\newcommand{\IfSymbol}{ite}
\newcommand{\AtSymbol}{!}

\newcommand{\AndSymbol}{$\wedge $}
\newcommand{\OrSymbol}{$ \vee $}
\newcommand{\NotSymbol}{$ \neg $}
\newcommand{\ImpliesSymbol}{$ \impl $}
\newcommand{\AddSymbol}{+}
\newcommand{\NegSymbol}{-}
\newcommand{\MulSymbol}{$ \times $}
\newcommand{\EqSymbol}{==}
\newcommand{\NeqSymbol}{$ \neq $}
\newcommand{\LeqSymbol}{$ \leq $}
\newcommand{\GeqSymbol}{$ \geq $}
\newcommand{\LeSymbol}{$ < $}
\newcommand{\GeSymbol}{$ > $}

\newcommand{\AndText}{and}
\newcommand{\OrText}{or}
\newcommand{\NotText}{not}
\newcommand{\ImplText}{implies}
\newcommand{\AddText}{add}
\newcommand{\MulText}{mul}
\newcommand{\EqText}{$==$}
\newcommand{\NeqText}{$!=$}
\newcommand{\LeqText}{$<=$}
\newcommand{\GeqText}{$>=$}
\newcommand{\LeText}{$<$}
\newcommand{\GeText}{$ > $}

\newcommand{\App}[2]{\ensuremath{#1 \, #2}}
\newcommand{\Lam}[3]{\ensuremath{\text{lam } (#1 : #2) \text{ . } #3}}
\newcommand{\Let}[4]{\ensuremath{\text{let } (#1 : #2) = #3 \text{ in } #4}}
%\newcommand{\Forall}[3]{\ensuremath{\forall (#1 : #2) \text{ . } #3}}
%\newcommand{\Exists}[3]{\ensuremath{\exists (#1 : #2) \text{ . } #3}}
\newcommand{\fAnd}[2]{\ensuremath{#1 \text{ \AndSymbol{} } #2}}
\newcommand{\fOr}[2]{\ensuremath{#1 \text{ \OrSymbol{} } #2}}
\newcommand{\fNot}[1]{\ensuremath{\text{\NotSymbol{} } #1}}
\newcommand{\If}[3]{\ensuremath{\text{if } #1 \text{ then } #2 \text{ else } #3}}
\newcommand{\Add}[2]{\ensuremath{#1 \text{ \AddSymbol{} } #2}}
\newcommand{\Mul}[2]{\ensuremath{#1 \text{ \MulSymbol{} } #2}}
\newcommand{\Eq}[2]{\ensuremath{#1 \text{ \EqSymbol{} } #2}}
\newcommand{\Neq}[2]{\ensuremath{#1 \text{ \NeqSymbol{} } #2}}
\newcommand{\Leq}[2]{\ensuremath{#1 \text{ \LeqSymbol{} } #2}}
\newcommand{\Geq}[2]{\ensuremath{#1 \text{ \GeqSymbol{} } #2}}
\newcommand{\Le}[2]{\ensuremath{#1 \text{ \LeSymbol{} } #2}}
\newcommand{\Ge}[2]{\ensuremath{#1 \text{ \GeSymbol{} } #2}}
\newcommand{\Seq}[2]{\ensuremath{[#1, ..., #2]}}
\newcommand{\elReal}{\ensuremath{r}}
\newcommand{\elEReal}{\ensuremath{p}}
\newcommand{\elNat}{\ensuremath{i}}
\newcommand{\elBool}{\ensuremath{b}}
\newcommand{\At}[2]{\ensuremath{#1 \text{ \AtSymbol{} } #2}}
%\newcommand{\hLam}[3]{\ensuremath{\text{lam } (#1 : #2) \text{ . } #3}}


% contexts
\newcommand{\polCtx}{P}
\newcommand{\forallPol}{+}
\newcommand{\existsPol}{-}
\newcommand{\hNetCtx}{N}
\newcommand{\hVarCtx}{\Sigma}
\newcommand{\hRandCtx}{Q}
\newcommand{\lNetCtx}{M}
\newcommand{\lInputVarCtx}{I}
\newcommand{\lOutputVarCtx}{O}
\newcommand{\semCtx}{\hNetCtx, \hRandCtx, \hVarCtx}

% types
\newcommand{\hTypeRel}[3]{#1 \Vdash #2 : #3}
\newcommand{\hcTypeRel}[2]{\hTypeRel{\Xi,\Delta}{#1}{#2}}
\newcommand{\hTypeRelp}[3]{#1 \Vdash #2 :^p #3}
\newcommand{\hcTypeRelp}[2]{\hTypeRelp{\Xi,\Delta}{#1}{#2}}
\newcommand{\hcNetCtx}{\Xi}
\newcommand{\hcVarCtx}{\Delta}
\newcommand{\haTypeRel}{\hcTypeRel{e}{\tau}}

\newcommand*{\validForm}[2][\hcNetCtx,\hcVarCtx]{#1 \Vvdash  #2}

\newcommand{\lTypeRel}[2]{#1 \Vdash #2}
\newcommand{\laTypeRel}{\lTypeRel{\lNetCtx}{e}}
\newcommand{\cTypeRel}{\lTypeRel{\Xi}{w}}

%grammar
\newcommand{\grammarItem}[1]{#1}
\newcommand{\typeClass}{\grammarItem{\tau}}
\newcommand{\exprClass}{\grammarItem{e}}
\newcommand{\opClass}{\grammarItem{op}}
\newcommand{\identClass}{\grammarItem{x}}
\newcommand{\netClass}{\grammarItem{f}}

\newcommand{\progClass}{\grammarItem{prog}}
\newcommand{\queryClass}{\grammarItem{query}}
\newcommand{\arithClass}{\grammarItem{arith}}
\newcommand{\compareClass}{\grammarItem{comp}}
\newcommand{\conjClass}{\grammarItem{conj}}
\newcommand{\inputVarClass}{\grammarItem{inputVar}}
\newcommand{\outputVarClass}{\grammarItem{outputVar}}

%rules
%%%% Rule label %%%%%
\newcommand*{\rulelabel}[1]{{\normalfont \textbf{(#1)}}}

\newcommand*{\LJArithL}{\rulelabel{Arith-L}}
\newcommand*{\LJArithR}{\rulelabel{Arith-R}}
\newcommand*{\LJAxiom}{\rulelabel{Axiom}}
\newcommand*{\LJCut}{\rulelabel{Cut}}
\newcommand*{\LJCtrL}{\rulelabel{C-L}}
\newcommand*{\LJCtrLT}{\rulelabel{CL-T}}
\newcommand*{\LJCtrR}{\rulelabel{C-R}}
\newcommand*{\LJWeakL}{\rulelabel{W-L}}
\newcommand*{\LJWeakLT}{\rulelabel{WL}}
\newcommand*{\LJWeakRT}{\rulelabel{WR}}
\newcommand*{\LJWeakR}{\rulelabel{W-R}}
\newcommand*{\LJExchLT}{\rulelabel{XL-T}}
\newcommand*{\LJCoFixRule}{\rulelabel{CO-FIX}}
\newcommand*{\LJConjL}{\rulelabel{$\conj$-L}}
%\newcommand*{\LJConjLG}{\rulelabel{$\conj$-L-G}}
\newcommand*{\LJConjR}{\rulelabel{$\conj$-R}}
\newcommand*{\LJDisjL}{\rulelabel{$\disj$-L}}
%\newcommand*{\LJDisjLG}{\rulelabel{$\disj$-L-G}}
\newcommand*{\LJDisjR}{\rulelabel{$\disj$-R}}
\newcommand*{\LJAllL}{\rulelabel{$\forall$-L}}
%\newcommand*{\LJAllLG}{\rulelabel{$\forall$-L-G}}
\newcommand*{\LJAllR}{\rulelabel{$\forall$-R}}
\newcommand*{\LJExL}{\rulelabel{$\exists$-L}}
%\newcommand*{\LJExLG}{\rulelabel{$\exists$-L-G}}
\newcommand*{\LJExR}{\rulelabel{$\exists$-R}}
\newcommand*{\LJImplL}{\rulelabel{$\to$-L}}
%\newcommand*{\LJImplLG}{\rulelabel{$\to$-L-G}}
\newcommand*{\LJImplR}{\rulelabel{$\to$-R}}
\newcommand*{\LJNegR}{\rulelabel{$\neg$-R}}
\newcommand*{\LJNegL}{\rulelabel{$\neg$-L}}

\newcommand*{\Ass}{\rulelabel{ASSUMP}}
\newcommand*{\Equi}{\rulelabel{EQUIV}}
\newcommand*{\IW}{\rulelabel{IW}}
\newcommand*{\IC}{\rulelabel{IC}}
\newcommand*{\EW}{\rulelabel{EW}}
\newcommand*{\EC}{\rulelabel{EC}}
\newcommand*{\EE}{\rulelabel{EE}}
\newcommand*{\SP}{\rulelabel{SPLIT}}
\newcommand*{\MX}{\rulelabel{MIX}}
\newcommand*{\pL}{\rulelabel{$p$-L}}
\newcommand*{\pR}{\rulelabel{$p$-R}}
\newcommand*{\oneL}{\rulelabel{$1$-L}}
\newcommand*{\oneR}{\rulelabel{$1$-R}}
\newcommand*{\zeroL}{\rulelabel{$0$-L}}
\newcommand*{\zeroR}{\rulelabel{$0$-R}}
\newcommand*{\botL}{\rulelabel{$\bot$-L}}
\newcommand*{\topR}{\rulelabel{$\top$-R}}
\newcommand*{\topL}{\rulelabel{$\top$-L}}
\newcommand*{\monL}{\rulelabel{$\conmul $-L}}
\newcommand*{\monR}{\rulelabel{$\conmul $-R}}
\newcommand*{\impL}{\rulelabel{$\ediv$-L}}
\newcommand*{\impR}{\rulelabel{$\ediv$-R}}
\newcommand*{\sandL}{\rulelabel{$\&^p$-L}}
\newcommand*{\sandLl}{\rulelabel{$\&^p$-L1}}
\newcommand*{\sandLr}{\rulelabel{$\&^p$-L2}}
\newcommand*{\orL}{\rulelabel{$\psum{p}$-L}}
\newcommand*{\andR}{\rulelabel{$\phsum{p}$-R}}
\newcommand*{\andRi}{\rulelabel{$\phsum{\infty}$-R}}
\newcommand*{\sorRl}{\rulelabel{$\psum{p}$-R1}}
\newcommand*{\sorRr}{\rulelabel{$\psum{p}$-R2}}
\newcommand*{\cut}{\rulelabel{CUT}}
\newcommand*{\comA}{\rulelabel{A-COM}}
\newcommand*{\comM}{\rulelabel{M-COM}}

%Sequents 
\newcommand{\bempty}[0]{\emptyset}
\newcommand{\eHyp}{\mathbb{I}}
%\newcommand*{\Hyp}{\mathcal{H}}
\newcommand*{\AssumsEnv}{\Gamma}
\newcommand*{\hsequentPDL}[2]{\Hyp \ | \ #1  \vdash #2}
\newcommand*{\ssequentPDL}[1]{\Hyp \ | \ #1 }
\newcommand*{\tsequentPDL}[1]{\Hyp }
\newcommand*{\csequentPDL}[4]{\Hyp \ | \ #1  \rightarrow #2 \ | \ #3  \vdash #4 }
\newcommand*{\sequentPDL}[2]{#1  \vdash #2}

\newcommand*{\sequentTt}[2]{ #1 \vdash #2}

\newcommand*{\sequentTf}[2]{ #1 \Vdash #2}

\newcommand*{\fsequentPDL}[3]{ #1  \xrightarrow{#2} #3}

\newcommand*{\psequentPDL}[3][\Sigma]{#1 \ | \ #2  \vdash #3}

%\newcommand*{\trail}[0]{2\textbackslash}
\newcommand*{\pen}[0]{\circ}
%Machine learning 
\newcommand{\losssymbol}{\mathcal{L}}


\newcommand{\setAtomsIn}{\mathbf{A}^{\mathrm{in}}}
\newcommand{\atomIn}{A^{\mathrm{in}}}
\newcommand{\atomOut}{A^{\mathrm{out}}}

\newcommand{\extOracle}{\mathsf{ext}}
\newcommand{\sampler}{\mathsf{samp}}
\newcommand{\boolReal}{\gamma}
\newcommand{\pfinder}{s}
\newcommand{\rfinder}{b}
